ABot-OCR Technical Report

We introduce ABot-OCR, an end-to-end vision-language model that transcribes a page image directly into clean Markdown in a single forward pass. By doing so, our approach completely eliminates the need for brittle modular orchestration. To maximize parsing fidelity, we develop a dedicated data engine to provide large-scale, structurally consistent supervision. Furthermore, we propose Decoupled Heterogeneous Document Optimization, a structure-constrained reinforcement learning method that sharpens textual accuracy and strictly enforces markup well-formedness beyond supervised fine-tuning alone. Extensive evaluations demonstrate the superior performance of our framework. On the OmniDocBench v1.5 and v1.6 benchmarks, ABot-OCR achieves state-of-the-art scores of 92.81 and 93.30 among all end-to-end systems, substantially narrowing the performance gap relative to strong pipeline baselines. Finally, comprehensive multilingual text recognition across ten diverse languages further confirms the robust generalizability of ABot-OCR.

==> data2.tex <==
\providecommand{\etal}{et al.}
\providecommand{\argmax}{\operatornamewithlimits{arg\,max}}
\providecommand{\Lev}{\operatorname{Lev}}
\providecommand{\KL}{\operatorname{KL}}
\providecommand{\clip}{\operatorname{clip}}
\providecommand{\Rtext}{R_{\text{text}}}
\providecommand{\Rformula}{R_{\text{formula}}}
\providecommand{\Rtable}{R_{\text{table}}}
\providecommand{\Rstruct}{R_{\text{struct}}}




\section{Data Engine}

The performance ceiling of end-to-end OCR models is primarily determined by the coverage, informativeness, and annotation accuracy of the training data. Existing data engines often organize data along a ``difficulty'' scalar and rely on absolute declarative annotations, which introduces two systemic issues:

\begin{itemize}
    \item The most valuable hard examples for model improvement are often the least reliable under automatic annotation (annotation paradox);
    \item The difficulty scalar obscures systematic failures of the model across different error types (error black-box).
\end{itemize}

To address these issues, we propose the \textbf{Diagnose-Verify (DV) Data Engine}, spanning data stratification, cleaning, annotation, hard example mining, and synthetic data generation. Its design is guided by two principles, each targeting one of the above problems:

\begin{itemize}
    \item \textbf{Error-Diagnosis First (addresses the ``error black-box'')}: Organize data by error type rather than difficulty scalar, explicitly decomposing systematic model failures for targeted data augmentation (cf. \S2.1).
    \item \textbf{Verifiable Supervision First (addresses the ``annotation paradox'')}: High-value hard examples do not rely on absolute human annotations but gain confidence through multi-model consistency and structural validity—``multi-source self-consistency'' replaces ``absolute correctness'' as the inclusion criterion (cf. \S2.2).
\end{itemize}

\subsection{Data Stratification Strategy }

The root of the ``error black-box'' problem lies in compressing different types of failures—table misalignment, character confusion, reading order errors, and format inconsistencies—into a single difficulty scalar. This makes it impossible to determine which error types the model systematically fails on, preventing targeted data reinforcement. We replace the difficulty scalar with \textbf{error-type distribution} as the data organization axis, making the black-box explicit.

To obtain an operational set of error types, we analyzed failure cases of \texttt{PaddleOCR\_VL}, \texttt{FireOCR}, and \texttt{MinerU2.5} on large-scale real PDFs. Key failures were consistently categorized into four types:

\begin{itemize}
    \item \textbf{Structural Errors}: Table row/column misalignment, missing formula alignment symbols, disrupted list hierarchy.
    \item \textbf{Recognition Errors}: Character misrecognition, visually similar character confusion.
    \item \textbf{Relational Errors}: Reading order errors, caption-figure mismatches, cross-page relationship breaks.
    \item \textbf{Format Errors}: Semantically equivalent but differently expressed content (HTML, Markdown, LaTeX, etc.).
\end{itemize}

This classification provides a clear organizational axis for subsequent cleaning, annotation, and hard example mining, allowing targeted improvement on the model's weaknesses.

\subsection{Data Cleaning and Multi-Dimensional Verification Framework}

The ``annotation paradox'' arises because the hard examples most critical for model learning are often the least reliable under single-source automatic annotation. The key insight of the Multi-Dimensional Verification Framework (MVF) is that OCR outputs are highly structured (LaTeX compilable, HTML/Markdown parsable, syntactic trees formally verifiable, layout geometrically mappable to the original image). Consequently, supervision confidence need not depend on ``agreement with human annotation'' but can be derived from ``multi-source consistency + structural validity.'' Structural evidence thus replaces absolute labels as the entry criterion for training hard examples.

The MVF consists of four orthogonal verification dimensions, each corresponding to one of the error types identified in \S2.1:

\begin{itemize}
    \item \textbf{Structural Consistency Verification (Structural Errors)}: Uses parsers/compilers to check compilability (LaTeX formulas, HTML tables) and structural closure (balanced brackets, proper \texttt{\textbackslash begin}/\texttt{\textbackslash end} environments, rowspan/colspan alignment, continuous list levels). Any failure flags a structural error.
    \item \textbf{Character Recognition Consistency Verification (Recognition Errors)}: Computes normalized edit distance across multiple model outputs at the character level. Segments below a threshold are considered multi-source consensus; high-distance segments are rewritten by a text expert model and re-voted.
    \item \textbf{Geometric Relationship Consistency Verification (Relational Errors)}: Assesses the coverage of bounding boxes over non-empty regions and measures variance in reading order paths, including cross-column jumps.
    \item \textbf{Format Normalization Consistency Verification (Format Errors)}: Compares normalized candidate annotations in a uniform format, eliminating pseudo-differences and quantifying semantic consistency.
\end{itemize}

All dimensions are independent and traceable. Each sample's final disposition (accepted / queued for repair / rejected) is fully interpretable. Thus, training signals no longer rely on ``correctness'' but on \textbf{multi-source structural and consistency verification}, effectively resolving the annotation paradox at scale.

\subsection{Data Annotation and Expert Model Closed-Loop}

During annotation, expert models generate supervision signals for both large-scale unannotated PDFs and partially verified samples requiring repair. The annotation system follows a \emph{reliability-increasing, granularity-decreasing} principle to form a closed loop.

First, the PaddleOCR layout detection model analyzes PDF pages, identifying text blocks, formula blocks, and tables, and outputs element boundaries and types. Then, each element type is annotated by a corresponding expert model: text elements produce character-level annotations and quantify consistency; formula elements generate structured LaTeX or symbolic trees; table elements perform cell recognition, merge/split, and alignment correction. Finally, all outputs pass through the MVF again, ensuring verifiable, consistent, and high-quality training data. Format errors are normalized during cleaning. This process forms a continuous loop from layout detection to element-level annotation to character-level verification, supporting end-to-end automated OCR data construction.

\subsection{Hard Example Mining \& Synthetic Data Augmentation}

Data augmentation combines natural hard example mining with synthetic data generation to produce high-quality, comprehensive training datasets. Natural hard examples are sampled preferentially based on model weaknesses in structural, recognition, relational, and format errors (\texttt{ModelWeakness(e)}), then verified via MVF and repaired by expert models. Perturbations are applied according to error type: structural errors are modified via table cell merges/splits, formula alignment disturbances, and list hierarchy rearrangements; recognition errors receive scanning noise or character occlusion; relational errors are perturbed via multi-column rearrangement, cross-page cuts, and caption-figure distance adjustments. All enhanced samples pass MVF again, ensuring consistency and traceability, forming a natural data augmentation loop.

To cover rare long-tail structures, template-driven synthetic data generates complex layouts (rare tables, long formulas, deep nested lists, multi-lingual content), verified via MVF, format normalization, and VLM-based semantic auditing. Natural augmented samples and synthetic data jointly form the training data loop, producing high-fidelity, diverse, and difficulty-balanced datasets for end-to-end OCR models, while ensuring traceability, consistency, and system reliability.

\paragraph{Summary} The Diagnose-Verify data engine organizes data by error type, integrating MVF, expert model annotation, natural hard example mining, and synthetic data augmentation to produce training data with high reliability, coverage, and diversity. The closed-loop design ensures traceability and consistency, and the synergy of natural and synthetic data enhances dataset completeness, providing solid support for end-to-end OCR models in both structural parsing and semantic understanding.





==> data3.tex <==
\providecommand{\etal}{et al.}
\providecommand{\argmax}{\operatornamewithlimits{arg\,max}}
\providecommand{\Lev}{\operatorname{Lev}}
\providecommand{\KL}{\operatorname{KL}}
\providecommand{\clip}{\operatorname{clip}}
\providecommand{\Rtext}{R_{\text{text}}}
\providecommand{\Rformula}{R_{\text{formula}}}
\providecommand{\Rtable}{R_{\text{table}}}
\providecommand{\Rstruct}{R_{\text{struct}}}

\section{Data Engine}
\label{sec:data-engine}

As model architectures mature, performance gains in end-to-end document parsing are increasingly bottlenecked by training data quality and distributional coverage. Existing data pipelines, however, fail to jointly optimize distributional coverage, sample complexity, and annotation fidelity. MinerU2.5~\cite{mineru25} employs IMIC to mine hard examples, but inherent single-model bias often yields ``consistently incorrect'' pseudo-labels at the model's capability boundary, severely compromising supervision reliability. MinerU2.5-Pro~\cite{mineru25pro} explicitly addresses this ``annotation paradox'' via Cross-Model Consistency Verification (CMCV) and a Judge-and-Refine loop, yet its sample scheduling remains tethered to a unidimensional difficulty scalar (Easy/Medium/Hard). This unidimensional mapping entrenches an \emph{error attribution opacity} that conflates heterogeneous failure modes---such as table misalignment, character confusion, and reading-order discontinuity---while omitting explicit structural validity verification. FireOCR~\cite{fireocr} employs dual-indexing and filtering for data curation but relies on a single-pass accept/reject decision for repairs; this open-loop design lacks iterative refinement and perpetuates supervision distortion in hard-example regimes.

These limitations underscore the critical need for a unified data engine that systematically decouples error diagnosis, multi-dimensional cascade verification, and closed-loop repair. Building upon the multi-source verification paradigm of CMCV, we propose the \textbf{Diagnose--Verify--Repair Data Engine (DVR)}. The DVR architecture is fundamentally structured around three synergistic pillars:

\begin{itemize}[leftmargin=*]
  \item \textbf{Diagnose}: Replaces the single difficulty scalar with an error-type distribution, enabling explicit decomposition and precise attribution of model failures (Section~\ref{sec:stratification}).
  \item \textbf{Verify}: Architects a funnel-style L1/L2/L3 Multi-Dimensional Cascade Verification (MDCV) framework, transforming CMCV's single-stage consensus check into a progressive pipeline comprising rule filtering, orthogonal divergence measurement, and rendering arbitration, while concurrently generating a modality-level confidence vector (Section~\ref{sec:mdcv}).
  \item \textbf{Repair}: Establishes a dual-track closed loop spanning sample-level correction and distribution-level enhancement. The former employs modality-aware routing to dispatch samples to specialized expert models, enforcing secondary verification and three quality gates prior to dataset ingestion (Section~\ref{sec:sample-repair}). The latter executes targeted perturbation and template synthesis driven by error-type distributions, subjecting all augmented samples to MDCV cascade review for admission (Section~\ref{sec:dist-aug}).
\end{itemize}

The primary innovations of DVR are summarized as follows:

\begin{enumerate}[leftmargin=*]
  \item \textbf{Error-Type $\times$ Content-Modality Dual-Axis Framework}---Decouples diagnostic signals and routing decisions into two independent axes: the error-type axis governs data augmentation and distribution optimization, while the content-modality axis directs expert-driven repair. Both axes derive from the same fine-grained MDCV signals but operate along orthogonal dimensions, circumventing the attribution ambiguity and resource misallocation inherent in CMCV's unidimensional difficulty scalar.
  \item \textbf{Funnel-style MDCV with Three-Layer Orthogonal Divergence Measurement}---Introduces a structural divergence metric $D$ alongside established task-level consistency metrics (TEDS / CDM / edit distance), achieving orthogonal decoupling across character, geometric, and structural measurement spaces. The L3 layer further provides \emph{robust arbitration under rendering anomalies}: AST validity and grid closure checks remain operational even under partial rendering failures, bridging the verification blind spot of traditional render-then-verify paradigms on structurally damaged samples. The overall computation protocol adheres to the OmniDocBench~\cite{omnidocbench} evaluation specification, ensuring benchmark compatibility.
  \item \textbf{Sample- and Distribution-Level Closed-Loop Repair}---Mandatorily reroutes repaired samples through the L2/L3 verification pipeline and subjects them to three stringent quality gates---consensus confidence gain, Local Repair Edit Distance, and Render-and-Readback arbitration---mitigating risks of ``over-modification'' and ``pseudo-repair'' while guaranteeing distribution-level augmentation undergoes identical validation.
\end{enumerate}

\subsection{Error-Type-Driven Data Stratification}
\label{sec:stratification}

The error attribution opacity discussed above stems from the inability of a unidimensional difficulty scalar to disentangle heterogeneous failure modes. Samples with comparable difficulty scores frequently harbor fundamentally distinct underlying failure mechanisms---e.g., table structural misalignment, character confusion, cross-page logical breaks, or formatting inconsistencies. Sampling strategies anchored solely to this one-dimensional metric therefore obscure the model's specific capability bottlenecks, impeding precise error diagnosis and targeted data augmentation.

DVR consequently shifts the stratification paradigm from difficulty scalars to \textbf{error-type distributions}. Grounded in a systematic analysis of failure modes exhibited by PaddleOCR\_VL~\cite{paddleocrvl}, FireOCR~\cite{fireocr}, and MinerU2.5~\cite{mineru25} across large-scale real-world PDF parsing tasks, we formulate a taxonomy comprising four core error categories:

\begin{itemize}[leftmargin=*]
  \item \textbf{Structural Errors}: table row/column misalignment, omitted formula alignment tokens, and list hierarchy fragmentation.
  \item \textbf{Recognition Errors}: character- or word-level OCR misrecognition, token omission, and visually similar character confusion.
  \item \textbf{Relational Errors}: reading-order inversion, caption--figure pairing mismatch, and broken cross-page logical chains.
  \item \textbf{Formatting Errors}: representational inconsistencies or missing delimiters for identical semantic content across distinct rendering paradigms (e.g., HTML, Markdown, \LaTeX{}).
\end{itemize}

This taxonomy serves as the unifying coordinate system for the rest of the engine: it converts heterogeneous failure modes---previously obscured by difficulty scalars---into structured, diagnosable, routable, and repairable training signals. Each downstream stage anchors directly to one or more of these categories: cascade verification (Section~\ref{sec:mdcv}) reports per-category divergence; expert repair (Section~\ref{sec:sample-repair}) consumes the same diagnostic vector when routing to specialists; and distribution-level perturbation (Section~\ref{sec:dist-aug}) is parameterized by the empirical frequency of each error type on the validation set. The four-category space is thus simultaneously a diagnostic schema and an actionable routing key.

\subsection{Multi-Dimensional Cascade Verification Framework (MDCV)}
\label{sec:mdcv}

The fundamental tension of the annotation paradox lies in the fact that highly informative hard examples reside precisely at the model's capability boundary, where single-source pseudo-labeling is prone to systematic bias, inevitably distorting supervision signals. DVR's key insight is that document parsing outputs inherently embody strong structural priors: \LaTeX{} and HTML adhere to formal syntax rules, page layouts maintain geometric alignment with source images, and Abstract Syntax Trees (ASTs) encode strict hierarchical logic. Confidence estimation therefore need not rely exclusively on manual annotation; it can yield computable and traceable supervision evidence through a combination of multi-source cross-consensus and structural validity verification.

Guided by this insight, DVR establishes the \textbf{Multi-Dimensional Cascade Verification (MDCV)} framework. Extending CMCV's multi-model consistency paradigm, MDCV evolves into a funnel-style cascade comprising rule-based pre-filtering, multi-source consensus, and semantic arbitration. L1 executes lightweight rule filtering to discard invalid samples exhibiting image corruption or formatting anomalies; L2 introduces a structural divergence metric $D$ as an independent structural-layer measurement that complements multi-model cross-verification; L3 leverages a Render-and-Readback (R\&R) mechanism to conduct semantic arbitration through a render--reconstruct and secondary-recognition loop, while synchronously generating a modality-level confidence vector. The framework follows a strict L1$\rightarrow$L2$\rightarrow$L3 routing protocol, yielding three-state outcomes (\texttt{Pass}, \texttt{Pending}, or \texttt{Reject}). By deferring high-overhead multi-model inference and rendering readback until after lightweight pre-filtering, MDCV eliminates redundant computation on low-quality samples and substantially improves overall pipeline throughput.

\begin{itemize}[leftmargin=*]
  \item \textbf{L1 Lightweight Rule Filtering}: This layer executes preliminary validity checks on both raw images and accompanying annotations. It first assesses image integrity by filtering out low-level corruption artifacts such as blank pages, rendering crashes, or full-page gibberish. For samples carrying original annotations, it concurrently verifies structural validity (e.g., tag closure, AST parsability). The routing protocol is strict: image-level anomalies are immediately \texttt{Reject}ed (excluded from downstream computation and archived for long-tail failure mode analysis); samples with intact images but structurally invalid annotations are stripped of their labels and downgraded to unlabeled status before proceeding to L2; samples passing both checks are forwarded to L2 for multi-source cross-verification.

  \item \textbf{L2 Multi-Source Cross-Verification}: Samples cleared by L1 enter the consensus verification layer. The system invokes three complementary parsing models (PaddleOCR\_VL~\cite{paddleocrvl}, FireOCR~\cite{fireocr}, MinerU2.5~\cite{mineru25}) in parallel to generate multiple candidate outputs, quantifying divergence across three orthogonal dimensions: character-level edit distance $\text{ED}$, layout intersection-over-union $\text{IoU}$, and structural divergence $D$. The definition of $D$ adheres to OmniDocBench~\cite{omnidocbench} specifications: table parsing employs $1-\text{TEDS}$ to quantify structural consistency, while formula parsing leverages a $\text{CDM}+\text{AST}$ hybrid strategy, ensuring seamless integration with established benchmark evaluation protocols. After scale normalization and similarity transformation, these metrics are aggregated into a consensus confidence score
  \[
    C = w_1\!\cdot\!(1-\text{ED}) + w_2\!\cdot\!\text{IoU} + w_3\!\cdot\!(1-D),
    \qquad \textstyle\sum_i w_i = 1,
  \]
  with weights calibrated offline on a held-out validation set. L2 executes an efficient binary gating mechanism: samples satisfying $C \geq \tau$ are accepted (\texttt{Pass}); all non-compliant candidates are uniformly routed to L3. L2 itself does not produce \texttt{Pending} states---fine-grained assessment for boundary cases and modality-level confidence estimation are deferred to L3.

  \item \textbf{L3 Semantic Arbitration}: For samples failing L2, the system initiates a Render-and-Readback closed loop: candidate structured outputs are rendered into images, spatially aligned with the source document, and subjected to secondary recognition. The final arbitration synthesizes a multi-dimensional metric suite---tree edit distance, cell matching rate, numerical consistency, AST validity, and grid closure---to yield a definitive verdict. Crucially, AST validity and grid closure checks can be evaluated \emph{independently of the rendering pipeline}, bridging the verification blind spot of traditional render-then-verify paradigms on structurally damaged candidates. To sustain throughput under heavy loads, L3 employs asynchronous scheduling with hard-example prioritization, augmented by rendering cache and region-level crop reuse to minimize pipeline blocking. This layer yields \texttt{Pass}, \texttt{Pending}, or \texttt{Reject} decisions, while concurrently aggregating fine-grained signals into the modality-level confidence vector $\mathbf{c} = (c_{\text{text}}, c_{\text{formula}}, c_{\text{table}}, c_{\text{layout}})$, which governs the modality-aware expert routing in Section~\ref{sec:sample-repair}.
\end{itemize}

\noindent\textbf{Three-State Routing.} \texttt{Pass} samples are ingested directly into the training set. \texttt{Reject} samples are filtered out and archived in a failure mode analysis repository---L1-intercepted instances undergo manual auditing for long-tail distribution defects, while L3-intercepted instances drive offline calibration of arbitration thresholds and metric weights. \texttt{Pending} samples are routed to the expert repair closed loop detailed in Section~\ref{sec:sample-repair}.

MDCV thus establishes a dynamic alignment between verification depth and sample uncertainty: high-value hard examples are no longer discarded due to the absence of manual annotations. Instead, guided by a traceable cascade evidence chain, they are strategically routed to either high-fidelity training corpora or targeted repair pipelines, transcending the rigid ``all-or-nothing'' arbitration paradigm of conventional data pipelines.

\subsection{Sample-Level Repair: Modality Routing and Expert Closed-Loop}
\label{sec:sample-repair}

Samples routed to \texttt{Pending} by MDCV retain high training value but exhibit complex semantic ambiguities and localized structural defects that exceed the resolution capacity of automated arbitration, making them the core repair anchors of the data pipeline. To go beyond the decision boundaries of single-stage verification, DVR establishes a sample-level expert repair closed loop: the system leverages the L3-generated modality-level confidence vector $\mathbf{c}$ to pinpoint vulnerable modalities and integrates error-type diagnostic signals to formulate targeted correction strategies, dispatching \texttt{Pending} samples to domain-specialist models for localized refinement. Following repair, samples are re-ingested into MDCV for secondary cascade verification, ensuring high-value hard examples are preserved rather than discarded after a single arbitration failure. This mechanism instantiates a ``verify--repair--reverify'' iterative closed loop.

\begin{itemize}[leftmargin=*]
  \item \textbf{Modality-Aware Routing}: Each \texttt{Pending} sample carries the L3-generated modality-level confidence vector $\mathbf{c} = (c_{\text{text}}, c_{\text{formula}}, c_{\text{table}}, c_{\text{layout}})$, which quantifies parsing reliability across distinct content modalities. The system executes targeted dispatch by identifying the minimum confidence component ($\argmin_{m} c_m$), corresponding to the most error-prone modality. Samples exhibiting weaknesses in text, formula, table, or layout are routed to the corresponding domain-specialist model---OCR refinement, formula reconstruction, table structure restoration, and layout parsing experts respectively---achieving precise modality-to-expert alignment.

  \item \textbf{Local Correction Constraint}: Expert models adhere to a \emph{minimal modification} principle, targeting only the low-confidence regions diagnosed by MDCV for correction and structural reconstruction, while preserving verified high-confidence segments intact. This constraint mitigates hallucination noise and distributional drift induced by global rewriting, and enables precise quantification of repair deltas via the \textbf{Local Repair Edit Distance (RED)}. RED quantifies the state transition of a single expert model pre- and post-repair, operating \emph{orthogonally} to the structural divergence metric $D$ that characterizes multi-source consensus disagreement in L2 (Section~\ref{sec:mdcv}). RED acceptance thresholds are dynamically calibrated according to content modality and initial confidence scores; this adaptive gating bounds ``over-modification'' risk while preserving fault tolerance for complex structural reconstruction.

  \item \textbf{Secondary Verification Loopback}: Repaired samples are rerouted back into MDCV for L2 consensus recalculation and L3 semantic arbitration, rather than admitted directly to the training corpus. Three concurrent quality gates apply:
  \begin{enumerate}[label=(\roman*),leftmargin=*]
    \item \textbf{Confidence Gain}: the post-repair target-modality confidence must improve ($\Delta c_m > 0$), or the global consensus confidence must increase upon re-evaluation with the repaired candidate ($\Delta C > 0$).
    \item \textbf{Correction Magnitude Constraint}: RED must reside within its dynamically calibrated bounds, preventing over-modification and hallucination injection.
    \item \textbf{Structural Arbitration Pass}: the L3 Render-and-Readback arbitration must yield a \texttt{Pass} verdict.
  \end{enumerate}
  Admission to the training corpus requires simultaneous satisfaction of all three gates. Non-compliant samples undergo stratified routing based on the magnitude of confidence degradation, with persistently low-confidence instances channeled to manual inspection queues and archived in the failure mode analysis repository for offline diagnostics.

  \item \textbf{Quality Flywheel}: Samples clearing the quality gates are merged with MDCV-direct \texttt{Pass} samples, progressively expanding the high-fidelity training corpus. Concurrently, the error-type distribution aggregated from hard examples in the current iteration functions as an offline diagnostic signal that periodically informs the recalibration of the MDCV consensus threshold $\tau$ and rebalances the fine-tuning distributions of expert models. Through this mechanism, DVR establishes a self-iterative data flywheel of \emph{candidate generation $\rightarrow$ cascade verification $\rightarrow$ targeted repair $\rightarrow$ distributional feedback}, ensuring the data engine continuously adapts and scales alongside the underlying model's capability improvements.
\end{itemize}

\subsection{Distribution-Level Augmentation: Error-Driven Perturbation and Synthetic Validation}
\label{sec:dist-aug}

Real-world data inherently carries natural distributional noise but exhibits significant sparsity in long-tail and complex structural patterns. Synthetic data, conversely, can effectively target and augment these rare distributions but typically lacks robust automated quality verification. Beyond the sample-level flywheel established in Section~\ref{sec:sample-repair}, DVR therefore introduces a distribution-level augmentation mechanism that bridges this gap. Anchored to the four error-type weak regions defined in Section~\ref{sec:stratification}, this pipeline synergizes natural hard-example resampling with template-driven synthesis. The design draws inspiration from FireOCR~\cite{fireocr}'s rendering-based generation paradigm but overcomes its open-loop, one-shot acceptance limitation: by subjecting every augmented sample to MDCV cascade review and stringent quality gating, the framework ensures safe, controllable, and high-fidelity admission of synthetic distributions into the training corpus.

Before describing the perturbation strategy itself, we emphasize a critical decoupling: the \textbf{error-type axis} that drives distribution-level augmentation is strictly \emph{orthogonal} to the \textbf{content-modality axis} that governs sample-level expert routing in Section~\ref{sec:sample-repair}. The two axes derive from the same fine-grained MDCV signals but address different decisions---\emph{what to perturb} (error type) versus \emph{whom to dispatch to} (modality)---and this separation prevents attribution conflation and ensures precise diagnostic targeting.

Guided by this principle, the system offline-aggregates MDCV diagnostic signals along the error-type axis to derive a distribution-level sampling weight $\text{ModelWeakness}(e)$, computed over the validation set. This metric directly repurposes existing MDCV outputs: structural, recognition, relational, and formatting weaknesses are respectively quantified via AST validity and grid closure rates, character-level consistency, reading-order alignment scores, and a composite of L1 syntax pass rate with L3 rendering divergence. Conditioned on high-weight error regions, the system injects targeted perturbations---such as table topology restructuring, OCR noise simulation, cross-page logical re-segmentation, and markup language transposition. All augmented samples are rerouted through the MDCV cascade; only those yielding a \texttt{Pass} verdict are admitted to the training corpus, guaranteeing safe and high-fidelity distributional expansion.

On the synthetic-data front, DVR leverages a template-driven pipeline to systematically synthesize complex samples underrepresented in natural distributions---rare table topologies, long-range formulas, deeply nested lists, and multilingual mixed layouts. Following format normalization and structural parsing, all generated candidates are routed through MDCV to execute L2 multi-source consensus and L3 Render-and-Readback arbitration. Only candidates clearing the established quality gates are admitted to the training corpus, guaranteeing safe and controllable expansion of the data distribution.

\subsection*{Summary}

Putting these components together, DVR establishes a self-evolving data closed loop of \emph{diagnosis--verification--repair--feedback}, orchestrated by error-type distributions, gated by Multi-Dimensional Cascade Verification, and driven by dual iterative mechanisms---sample-level targeted repair and distribution-level synthetic augmentation. The engine not only ensures robust coverage of mainstream document parsing distributions but also systematically bridges the structural and semantic long-tails where models are most vulnerable. Through error-driven targeted perturbations and expert corrections, DVR transcends the attribution opacity of single-dimensional difficulty routing and resolves the supervision reliability bottleneck inherent in single-source pseudo-labeling.

%==============================================================================
%  References
%  TODO: replace placeholders with full bibliographic details, or use a .bib.
%==============================================================================
% \begin{thebibliography}{9}
%   \bibitem{mineru25}     MinerU2.5. \emph{[TODO: complete bibliographic details].}
%   \bibitem{mineru25pro}  MinerU2.5-Pro. \emph{[TODO: complete bibliographic details].}
%   \bibitem{fireocr}      FireOCR. \emph{[TODO: complete bibliographic details].}
%   \bibitem{omnidocbench} OmniDocBench. \emph{[TODO: complete bibliographic details].}
%   \bibitem{paddleocrvl}  PaddleOCR\_VL. \emph{[TODO: complete bibliographic details].}
% \end{thebibliography}

% \end{document}

==> data_v2.tex <==
\section{Data Engine}
\label{sec:data-engine}

% The performance upper bound of end-to-end OCR models is fundamentally constrained by the coverage, informativeness, and label reliability of the training corpora. Conventional data engines typically stratify data based on scalar difficulty scores and rely on absolute, declarative annotations. We identify two systemic shortcomings in this paradigm:
% \begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
% \item \textbf{The Annotation Paradox}: Samples that are most informative for model refinement are often the least reliable when subjected to automated labeling pipelines.
% \item \textbf{The Error Black-Box}: Aggregating failures into a singular difficulty score obscures the underlying failure modes, hindering targeted diagnostic improvements.
% \end{itemize}

% To address these limitations, we propose the Diagnose--Verify (DV) data engine, a holistic framework integrating data stratification, cleaning, annotation, hard-example mining, and synthetic data generation. The DV engine operates on two foundational principles:
% \begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
% \item \textbf{Error-Driven Diagnostics}: Moving beyond scalar difficulty, we organize data by error taxonomy to decompose systematic failure modes, thereby enabling targeted augmentation (\S\ref{sec:stratification}).
% \item \textbf{Verifiable Supervision}: We replace absolute human-ground-truth reliance with multi-source self-consistency and structural validity, ensuring high-value hard examples are accurately admitted into the training set (\S\ref{sec:mvf}).
% \end{itemize}

Modern end-to-end OCR formulations have shifted the performance bottleneck from architectural design to data scaling laws; the upper bound of text recognition accuracy is now fundamentally dictated by how effectively a data engine can manage data density, diversity, and label integrity. Conventional data management practices, however, typically employ a simplistic triage strategy: data is stratified based on raw error rates or confidence scores, and annotations are assumed to be static, unyielding truths. This conventional paradigm suffers from two self-limiting flaws:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{The Annotation Paradox}: Rare and long-tail data points are highly valuable because they can help the model break through its current performance bottlenecks. However, these specific samples are also the exact places where automated labeling tools make the most mistakes. Because of this contradiction, standard data pipelines often reject these high-value images simply due to low label confidence, creating a wasteful and vicious cycle.
\item \textbf{The Error Black-Box}: Traditional data engines group completely different types of mistakes into a single, uniform difficulty score. For example, they treat multi-oriented text, complex tables, and blurry historical scripts as if they were the same problem. This approach hides the true nature of the errors. Therefore, developers cannot diagnose whether a model failed because it could not locate the text or because it could not understand the language.
\end{itemize}

To address these challenges, we present the Diagnose--Verify (DV) data engine, a holistic ecosystem engineered to transform raw, noisy data streams into a highly curated, self-improving training corpus through synchronized stratification, filtration, and generative augmentation. The design philosophy of the DV engine revolves around two operational breakthroughs:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Diagnostic Decomposition}: We replace scalar grading with an explicit error taxonomy (\S\ref{sec:stratification}). By categorizing text-recognition failures into clear sub-domains (e.g., sensory degradation vs. syntactic ambiguity), the engine acts as an automated debugger, directing specialized synthetic data generation pipelines to actively fortify the model's weakest frontiers.
\item \textbf{Verifiable Consensus Consensus}: We shift the annotation paradigm from absolute, fragile single-source labels to a robust verification framework rooted in multi-experts self-consistency and cross-modal structural checks (\S\ref{sec:mvf}). This mechanism ensures that even the most ambiguous hard examples are assigned multi-dimensionally verified, reliable supervision before entering the optimization loop.
\end{itemize}

\vspace{0.5em}
\noindent
\begin{center}
  \includegraphics[width=0.88\textwidth]{figure/data_engine.png}
  \captionof{figure}{Schematic of our proposed data engine.}
  \label{fig:data_engine}
\end{center}
\vspace{0.8em}

% \subsection{Data Stratification Strategy}
% \label{sec:stratification}

% The error black-box phenomenon arises when heterogeneous failure modes---including table misalignment, character confusion, reading-order errors, and format inconsistencies---are collapsed into a univariate difficulty score.
% This compression masks the distribution of dominant error types and impedes targeted data reinforcement.
% Accordingly, the scalar difficulty axis is replaced by an error-type distribution.

% Failure cases of \texttt{PaddleOCR\_VL}, \texttt{Firered-OCR}, and \texttt{MinerU2.5} on large-scale document corpora motivate an operational taxonomy with four primary categories:
% \begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
%   \item \textbf{Structural errors:}
%     misalignment in table rows and columns, missing mathematical operators, and disrupted list hierarchies;
%   \item \textbf{Recognition errors:}
%     character misclassification and confusion among visually similar glyphs;
%   \item \textbf{Relational errors:}
%     incorrect reading order, caption--figure misalignment, and broken cross-page references;
%   \item \textbf{Format errors:}
%     markup variants (e.g., HTML, Markdown, \LaTeX) for semantically identical content.
% \end{itemize}

% This taxonomy provides a concrete framework for subsequent cleaning and mining, facilitating targeted data augmentation based on observed model vulnerabilities.

\subsection{Data Stratification Strategy}
\label{sec:stratification}

The error black-box phenomenon happens when traditional systems pack completely different types of mistakes into a single difficulty score. For instance, they group table misalignment, character confusion, reading-order errors, and formatting issues all together. This heavy compression is problematic because it hides the real distribution of the dominant error types. Therefore, developers cannot know which specific mistakes happen most often, making it impossible to perform targeted data reinforcement. To solve this issue, we replace the single scalar difficulty score with a detailed error-type distribution.

We carefully analyzed why popular OCR models like \texttt{PaddleOCR\_VL}, \texttt{Firered-OCR}, and \texttt{MinerU2.5} fail on large-scale document datasets. Based on these practical observations, we designed a clear taxonomy with four main error categories:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Structural errors}: This category includes misaligned rows and columns in tables, missing mathematical operators, and broken list hierarchies.
\item \textbf{Recognition errors}: This category covers character misclassification and confusion between visually similar characters or glyphs.
\item \textbf{Relational errors}: This group focuses on incorrect reading orders, misaligned captions and figures, and broken cross-page text references.
\item \textbf{Format errors}: This involves using different code variants, such as HTML, Markdown, or \LaTeX, to represent the exact same semantic content.
\end{itemize}

Ultimately, this taxonomy gives us a concrete and practical framework. It guides our subsequent data cleaning and hard-example mining. By knowing exactly where the model is vulnerable, we can now perform highly targeted data augmentation to fix its specific weaknesses.

% \subsection{Data Cleaning and Multi-Dimensional Verification Framework}
% \label{sec:mvf}

% The annotation paradox reflects a disconnect between learning utility and label reliability. Our Multi-dimensional Verification Framework (MVF) leverages the inherent structure of OCR outputs (e.g., compilable \LaTeX, parsable HTML, and geometric layout consistency) to ground supervision confidence in formal validity. Structural evidence, rather than mere declarative correctness, gates the inclusion of hard examples.

% The MVF comprises four orthogonal verification dimensions, aligned with our error taxonomy:
% \begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
% \item \textbf{Structural consistency}: Compilers and parsers verify formal syntax (e.g., balanced \LaTeX{} delimiters, matched \texttt{rowspan}/\texttt{colspan} in HTML tables).
% \item \textbf{Character recognition consistency}: We compute the normalized edit distance across multiple model outputs; consensus is verified through expert model rescoring for ambiguous spans.
% \item \textbf{Geometric relationship consistency}: We quantify bounding-box coverage and path variance to validate reading-order integrity.
% \item \textbf{Format normalization consistency}: Annotations are projected into a canonical representation to filter out spurious surface variations and quantify semantic agreement.
% \end{itemize}

% These dimensions provide interpretable dispositions (accept, repair, or reject) for each sample, alleviating the annotation paradox while maintaining data scale.

\subsection{Data Cleaning and Multi-Dimensional Verification Framework}
\label{sec:mvf}

The annotation paradox happens because the most useful training data is often the hardest to label correctly. To solve this problem, we developed the Multi-dimensional Verification Framework (MVF). Instead of just blindly trusting the text labels, MVF checks the internal structure of the OCR outputs to see if they make sense. For example, it checks if the \LaTeX{} code can compile successfully, if the table HTML code can be parsed, and if the geometric layout is consistent. We only allow hard examples to enter the training set if they pass these strict structural checks.

The MVF uses four independent check dimensions to verify data. These dimensions directly match our four error categories:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Structural consistency}: We use standard compilers and parsers to check the syntax. For instance, we verify if \LaTeX{} math delimiters are properly closed, and if HTML table rows and columns match perfectly.
\item \textbf{Character recognition consistency}: We compare the text outputs from multiple different OCR models and calculate how much they disagree. If a piece of text is too ambiguous, we pass it to a specialized expert model to make the final decision.
\item \textbf{Geometric relationship consistency}: We calculate the bounding box coordinates and text paths of the document. This math check helps us ensure that the reading order of the text flows naturally and correctly.
\item \textbf{Format normalization consistency}: We convert all raw annotations into a single, standardized format. This step helps us filter out minor coding variations and accurately check if different labels share the exact same meaning.
\end{itemize}

Ultimately, these four checks give us a clear action for every single data sample. The system will automatically decide to accept, repair, or reject the data. By using this method, we can successfully collect a massive amount of hard training data without introducing dirty or incorrect labels.

% \subsection{Data Annotation and Expert-Model Closed Loop}
% \label{sec:annotation}

% We utilize expert models to generate supervision for unannotated documents, following a pipeline characterized by increasing reliability and decreasing granularity. A layout detector (e.g., \texttt{PaddleOCR}) first segments pages into blocks (text, formula, table). Specialized experts then process each category: text blocks are transcribed with consistency scores, formula blocks are parsed into symbolic trees, and table blocks are reconstructed for alignment. All outputs undergo MVF screening to ensure verifiable consistency, creating an automated loop that minimizes manual intervention.

\subsection{Data Annotation and Expert-Model Closed Loop}
\label{sec:annotation}

We use specialized expert models to automatically label unlabeled documents. Our processing pipeline follows a clear order, working from the large layout structures down to the smallest text details. First, a layout detector like \texttt{PaddleOCR} divides the document page into different functional blocks, such as text paragraphs, formulas, and tables. Next, specialized expert models process each category separately. For text blocks, the model transcribes the words and calculates a consistency score. For formula blocks, the model parses the math symbols into a clean symbolic tree. For table blocks, the model reconstructs the rows and columns to ensure everything aligns perfectly. Finally, all these outputs must pass through our MVF screening system. This check ensures that every automated label is reliable and verified. Together, these steps create a completely automated loop that dramatically reduces the need for manual work.

% \subsection{Hard-Example Mining and Synthetic Data Augmentation}
% \label{sec:augmentation}

% Augmentation integrates natural hard-example mining with template-driven synthesis. We identify samples where model confidence is low across our four error categories, subsequently applying targeted perturbations (e.g., table structure noise, scan artifacts, column shuffling). Simultaneously, we generate synthetic data for long-tail layouts, followed by MVF screening and VLM-based semantic auditing. This hybrid approach ensures a balanced training distribution characterized by both high diversity and verifiable provenance.

% \paragraph{Summary}
% The Diagnose--Verify engine synthesizes error-aware stratification, multi-dimensional verification, and expert-driven closed-loop annotation. This design significantly enhances the reliability and diversity of training corpora, providing a scalable solution for robust end-to-end document parsing.

\subsection{Hard-Example Mining and Synthetic Data Augmentation}
\label{sec:augmentation}

Our data augmentation strategy combines natural hard-example mining with template-driven data synthesis. First, we find real data samples where the model shows low confidence in any of our four error categories. Once we identify these weak spots, we apply targeted changes to the images. For instance, we deliberately add table structure noise, simulate scan artifacts, or shuffle columns. At the same time, we use templates to automatically generate synthetic data for rare, long-tail document layouts. Finally, all newly generated data must pass through our MVF screening and a VLM-based semantic check. This hybrid approach ensures our training dataset is perfectly balanced. It provides both high data diversity and completely verifiable quality.

\paragraph{Summary}
In short, the Diagnose--Verify engine brings together error-driven stratification, multi-dimensional verification, and an automated expert annotation loop. This holistic design greatly improves both the reliability and the diversity of the training data. Ultimately, it provides a highly scalable solution for building robust, end-to-end document parsing models.

==> data_v3.tex <==
\section{Data Engine}
\label{sec:data-engine}

Modern end-to-end OCR formulations have shifted the performance bottleneck from architectural design to data scaling laws; the upper bound of text recognition accuracy is fundamentally dictated by how effectively a data engine manages data density, diversity, and label integrity. Conventional data management practices, however, typically employ a simplistic triage strategy: data is stratified based on raw error rates, and annotations are assumed to be static, unyielding truths. This conventional paradigm suffers from two self-limiting flaws: \textit{Label Instability in Long-Tail Distributions}, where rare, high-value edge cases are prematurely discarded due to automated labeling noise, and \textit{Monolithic Error Aggregation}, where distinct error modalities (e.g., complex tables vs. degraded scripts) are collapsed into a single, uninformative scalar difficulty score.

To resolve these challenges, we introduce the \textbf{Taxonomy-Guided Verification (TGV)} data engine, a holistic ecosystem engineered to transform raw, noisy document streams into a highly curated, self-improving training corpus. As illustrated in Fig.~\ref{fig:data-engine}, the TGV engine operationalizes data engineering into three interconnected, synergistic pillars: multi-dimensional data cleaning, automated expert-in-the-loop annotation, and diagnostic hard-example mining.

\vspace{0.5em}
\noindent
\begin{center}
  \includegraphics[width=0.88\textwidth]{figure/data_engine_v2.png}
  \captionof{figure}{Schematic architecture of the proposed Taxonomy-Guided Verification (TGV) data engine.}
  \label{fig:data-engine}
\end{center}
\vspace{0.8em}

% =========================================================================
% Pillar 1: Data Cleaning
% =========================================================================
\subsection{Data Cleaning via Multi-Dimensional Verification}
\label{sec:data-cleaning}

To guarantee label integrity without discarding valuable hard examples, we propose the Multi-dimensional Verification Framework (MVF). Rather than relying solely on naive confidence scores, MVF evaluates the intrinsic structural and syntactic validity of candidate text representations. By executing cross-modal consistency checks, the framework automatically decides whether to accept, repair, or reject each data sample, effectively filtering out corrupted data while preserving challenging linguistic layouts.

The cleaning pipeline operates across three orthogonal verification dimensions, directly counteracting downstream parsing anomalies:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Structural Rule-Checking}: Syntactic validity is enforced using deterministic compilers and parsers. For instance, \LaTeX\ mathematical formulas are checked for properly closed delimiters, and HTML table tokens are parsed to ensure matrix structural integrity.
\item \textbf{Geometric Relationship Constraints}: Bounding box coordinates and reading paths are mathematically cross-examined. This spatial validation guarantees that the logical flow of text complies with natural reading orders, pruning out chaotic layout segments.
\item \textbf{Format Normalization Consistency}: Raw text strings are unified into a standardized representation. This step eliminates minor syntactic variants (e.g., Markdown vs. HTML vs. \LaTeX\ syntax for identical content), allowing the engine to isolate genuine text discrepancies from superficial encoding differences.
\end{itemize}

% =========================================================================
% Pillar 2: Data Annotation
% =========================================================================
\subsection{Automated Data Annotation and Expert Consensus}
\label{sec:data-annotation}

To bypass manual labeling bottlenecks and mitigate label instability in long-tail samples, the TGV engine establishes a fully automated, multi-expert annotation closed loop. Unlabeled multi-page documents are processed via a hierarchical ``coarse-to-fine'' strategy, where structural layouts are decomposed before fine-grained textual transcriptions are executed. 

The annotation workflow is structured as follows:
\begin{enumerate}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Hierarchical Layout Decomposition}: A robust layout detector (e.g., \texttt{PaddleOCR}) first segments the document page into functional regions, separating standard text paragraphs, isolated mathematical expressions, and tabular blocks.
\item \textbf{Specialized Expert Transcription}: Each isolated region is routed to a specialized expert model. Text blocks are transcribed into standard strings; formula blocks are parsed into symbolic expression trees; and tables are reconstructed into aligned structural matrices.
\item \textbf{Consensus Verification}: For ambiguous or highly complex regions where specialized models exhibit high variance, a cross-model consensus mechanism is triggered. The system calculates token-level disagreement across multiple models, invoking an advanced visual-language model (VLM) to arbitrate final supervision when necessary. 
\end{enumerate}
The resulting labels are then fed back into the MVF (\S\ref{sec:data-cleaning}) for final quality gating, ensuring that the training set scales with zero injection of dirty annotations.

% =========================================================================
% Pillar 3: Data Mining
% =========================================================================
\subsection{Diagnostic Hard-Example Mining and Target Augmentation}
\label{sec:data-mining}

The core mechanism for model self-improvement within the TGV engine relies on deconstructing monolithic error aggregation. By analyzing why prominent document parsers (e.g., \texttt{PaddleOCR\_VL}, \texttt{Firered-OCR}, and \texttt{MinerU2.5}) fail on large-scale corpora, we replace scalar grading with an explicit four-tiered error taxonomy: \textit{Structural errors} (table misalignments), \textit{Recognition errors} (character confusion), \textit{Relational errors} (reading order failures), and \textit{Format errors} (code representation variants).

This taxonomy acts as a diagnostic debugger to drive our hard-example mining and generative augmentation loops:
\begin{itemize}[leftmargin=1.4em, itemsep=0.2em, topsep=0.3em]
\item \textbf{Targeted Hard-Example Mining}: The data engine tracks the model's posterior probability distributions across the four error tiers. Samples exhibiting high epistemic uncertainty or localized low confidence are mined as critical training data.
\item \textbf{Generative Layout Augmentation}: To actively fortify the model's weakest frontiers, mined hard examples undergo targeted transformations. We inject synthetic structural noise, simulate physical scan artifacts, or perform structural column shuffling based on the diagnosed error profiles.
\item \textbf{Template-Driven Long-Tail Synthesis}: For extremely rare or out-of-distribution document styles, template-based synthesis pipelines are deployed to populate low-density data regions.
\end{itemize}
All mined and augmented samples must pass through a VLM-backed semantic check and the MVF gating system, yielding a perfectly balanced training distribution characterized by high diversity and verifiable quality.

==> method.tex <==
% This file is intended to be included from `paper.tex` via \input.

\providecommand{\etal}{et al.}
\providecommand{\argmax}{\operatornamewithlimits{arg\,max}}
\providecommand{\Lev}{\operatorname{Lev}}
\providecommand{\KL}{\operatorname{KL}}
\providecommand{\Rtext}{R_{\text{text}}}
\providecommand{\Rformula}{R_{\text{formula}}}
\providecommand{\Rtable}{R_{\text{table}}}
\providecommand{\Rstruct}{R_{\text{struct}}}

\section{Methodology}
\label{sec:method}

\subsection{Problem Formulation}
\label{sec:problem}

We treat document parsing as an end-to-end image-to-Markdown generation
problem. Given a page image $I \in \mathbb{R}^{H \times W \times 3}$, the
model $\pi_\theta$ produces a target sequence $y = (y_1, \dots, y_T)$ that
conforms to a Markdown subset comprising plain text, heading hierarchy,
lists, tables expressed in HTML, display/inline formulas in \LaTeX, and an
implicit reading order over these elements.

Bounding-box predictions are emitted as plain text using the coordinate-token
convention of Qwen-VL \citep{bai2023qwen}. The whole system is therefore a
single autoregressive map $I \mapsto y$, and different tasks differ only in
the prompt token that conditions $\pi_\theta$.

Across the three training stages described below, we jointly optimize the
supervised likelihood and, in the final stage only, an expected reward:
\begin{equation}
\pi^{\star} \;=\; \argmax_{\theta}\;
  \mathbb{E}_{(I, y^{\star}) \sim \mathcal{D}}\!\left[\log \pi_\theta(y^{\star} \mid I)\right]
  \;+\; \lambda\, \mathbb{E}_{I \sim \mathcal{D}}\!\left[\mathcal{R}\!\left(\pi_\theta(I)\right)\right],
\label{eq:overall}
\end{equation}
where $\mathcal{R}(\cdot)$ aggregates the rule-based rewards introduced in
\Cref{sec:stage3}. Stages~1 and~2 set $\lambda = 0$ and optimize the
likelihood term alone; Stage~3 sets $\lambda > 0$ and optimizes the reward
term via GDPO. All three stages share the same backbone, initialized from
Qwen3-VL-2B-Instruct \citep{qwen3vl2025}.

\subsection{Three-Stage Training Pipeline}
\label{sec:overview}

A natural baseline is to fine-tune a strong VLM directly on
\textit{(page image, full Markdown)} pairs. In our preliminary experiments
this single-step recipe failed in two recurring ways.

The first is \emph{structural hallucination}: tables with inconsistent row
widths, unclosed \texttt{\$\$} pairs, and HTML tags opened but never closed.
The token-level loss does not penalize these errors because they are
sequence-level properties---the cross-entropy can converge to a low value
while the generated Markdown remains structurally invalid.

The second is \emph{gradient interference}: the signals required for
locating glyphs, recognizing them, and serializing the page into Markdown
compete with one another during optimization, and accuracy on long-tail
content---rare formulas, complex table layouts---degrades sharply.

These observations \citep{fireredocr2025} motivate decoupling these
capabilities before integrating them. Accordingly, our training recipe
follows the three-stage pipeline illustrated in
\Cref{fig:three_stage_pipeline}:

\begin{itemize}[leftmargin=1.6em, itemsep=0.4em, topsep=0.4em]
  \item \textbf{Stage 1 -- Multi-task pre-alignment.} Cross-entropy SFT on
    four visually heterogeneous subtasks (text spotting, formula recognition,
    table recognition, layout analysis) covering the local and global
    perception primitives needed for page-level parsing.
  \item \textbf{Stage 2 -- End-to-end specialization.} Cross-entropy SFT on
    \textit{(page image, normalized Markdown)} pairs. The model learns to
    compose the Stage~1 primitives into a single coherent output.
  \item \textbf{Stage 3 -- Multi-reward RL refinement.} Rule-based rewards
    on text fidelity and structural well-formedness are optimized with GDPO
    \citep{liu2026gdpo}, a multi-reward variant of GRPO
    \citep{shao2024deepseekmath} that avoids advantage collapse.
\end{itemize}

The remainder of this section presents each stage in detail
(\Cref{sec:stage1,sec:stage2,sec:stage3}).

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/method.jpg}
    \caption{Overview of the proposed three-stage training pipeline for document-to-Markdown parsing. Stage~1 performs multi-task pre-alignment on text spotting, formula recognition, table recognition, and layout analysis to build fine-grained visual and structural perception. Stage~2 specializes the model with end-to-end supervised fine-tuning on normalized page-to-Markdown pairs. Stage~3 further refines the policy with GDPO using rule-based rewards for text fidelity, formula correctness, table integrity, and structural closure.}
    \label{fig:three_stage_pipeline}
\end{figure}

\subsection{Stage 1: Multi-task Pre-alignment}
\label{sec:stage1}

A general-purpose VLM has only a coarse understanding of documents:
web-scale pretraining does not select for the fine-grained pixel-to-character
alignment that OCR requires. Stage~1 jointly trains four complementary
supervisions through the same network---routed by a task-specific
prompt token, with no task-specific heads
\citep{bai2023qwen, chen2024internvl}---so that by the end of training the
visual encoder has internalized representations Stage~2 can compose.
The Stage~1 dataset is
$\mathcal{D}_{\text{S1}} = \mathcal{D}_{\text{spot}} \cup \mathcal{D}_{\text{formula}} \cup \mathcal{D}_{\text{table}} \cup \mathcal{D}_{\text{layout}}$,
with the four tasks defined below.

\paragraph{Text spotting.} Given a full page and prompt token \texttt{<spot>},
the model emits sequences of the form
\[
\texttt{<|box\_start|>(x1,y1),(x2,y2)<|box\_end|>text\_content}
\]
following Qwen-VL's coordinate-token convention \citep{bai2023qwen}. Spotting
is the most demanding task for visual perception---the network must
localize text regions, recognize their content, and emit pixel-accurate
coordinates within a single sequence---and serves as the foundation for the
subsequent layout-aware tasks.

\paragraph{Formula recognition.} The input is either a cropped formula
region or a full page with a region-of-interest prompt; the target is a
normalized \LaTeX{} string covering inline, display, and multi-line numbered
formulas.

\paragraph{Table recognition.} Given a cropped table image, the model
outputs a normalized HTML table of the form
\verb|<table><tr><td>...</td></tr></table>|. We use HTML uniformly, even
for tables expressible as Markdown pipes: it expresses \texttt{rowspan} and
\texttt{colspan} natively, and adopting a single grammar allows Stage~3's
structural reward (\Cref{sec:stage3}) to be defined over one syntax rather
than two.

\paragraph{Layout analysis.} Given a full page and the prompt token
\texttt{<layout>}, the model produces a reading-order-sorted sequence of
region boxes paired with a region type drawn from
\{\textit{title, text, table, figure, formula, footer, $\dots$}\}:
\[
\texttt{<|box\_start|>(x1,y1),(x2,y2)<|box\_end|><type>title</type>}.
\]

\medskip
The four tasks decompose naturally into two groups: spotting and layout
provide \emph{global} spatial supervision over the page, while formula and
table recognition provide \emph{local} structural supervision over their
respective content types. These two forms of supervision are complementary
in the visual encoder.

Stage~1 minimizes the standard autoregressive cross-entropy
\begin{equation}
\mathcal{L}_{\text{S1}}(\theta) \;=\; -\, \mathbb{E}_{(I, c, y) \sim \mathcal{D}_{\text{S1}}}
\!\left[ \sum_{t=1}^{|y|} \log \pi_\theta(y_t \mid y_{<t},\, I,\, c) \right],
\label{eq:l-stage1}
\end{equation}
where $c \in \{\texttt{<spot>}, \texttt{<formula>}, \texttt{<table>}, \texttt{<layout>}\}$
is the task-routing prompt. Minibatches sample the four tasks at ratio
$\rho_{\text{spot}} : \rho_{\text{formula}} : \rho_{\text{table}} : \rho_{\text{layout}} = 3{:}2{:}2{:}3$:
a roughly inverse-size weighting that oversamples the smaller formula and
table corpora, while allocating the largest combined share to spotting and
layout, which operate over full pages and drive global perception.

By the end of Stage~1, the visual encoder has internalized the perception
primitives---glyph-level reading, layout understanding, and formula and
table parsing---that Stage~2 will compose into Markdown, without needing
to relearn them while simultaneously learning serialization.

\subsection{Stage 2: End-to-End Document Parsing}
\label{sec:stage2}

Stage~1 establishes the model's \emph{local} capabilities; Stage~2 trains
it to integrate them, mapping a single page image to a single Markdown
string that captures all of its content. The primary challenge becomes
structural well-formedness: closed tags, consistent heading depths, and
properly delimited math. Cross-entropy remains the objective; reward-based
shaping is reserved for Stage~3.

Let $\mathcal{D}_{\text{S2}} = \{(I^{\text{page}}_i, M^{\star}_i)\}_{i=1}^{N_2}$.
The ground-truth Markdown $M^{\star}$ is produced by a strict normalization
pipeline. The relevant invariants are:
\begin{itemize}[leftmargin=1.4em, itemsep=0.15em, topsep=0.3em]
  \item Display math is delimited by \verb|$$ ... $$|, inline math by
    \verb|$ ... $|.
  \item All tables are HTML, irrespective of whether they contain merged
    cells, so that Stage~3's table reward operates over a single grammar.
  \item Reading order follows the visual layout: in multi-column pages,
    columns are emitted left-to-right with full column completion before
    advancing; figure captions are tied to their figures, not to surrounding
    paragraphs.
  \item Heading depth is expressed via \verb|#|, \verb|##|, \verb|###|, with
    no skips (no \verb|#| followed directly by \verb|###|).
\end{itemize}
These invariants are seemingly minor but consequential: most of the
reward-shaping decisions in Stage~3 derive their structure from them.
The training objective is
\begin{equation}
\mathcal{L}_{\text{S2}}(\theta) \;=\; -\, \mathbb{E}_{(I^{\text{page}}, M^{\star}) \sim \mathcal{D}_{\text{S2}}}
\!\left[ \sum_{t=1}^{|M^{\star}|} \log \pi_\theta\!\left(M^{\star}_t \mid M^{\star}_{<t},\, I^{\text{page}}\right) \right].
\label{eq:l-stage2}
\end{equation}
Training resumes from the Stage~1 checkpoint. We freeze the visual encoder
for the remainder of training and update only the language model and the
cross-modal projector: by this point the encoder has internalized the
perception primitives acquired in Stage~1, and the dominant remaining
task---composing them into well-formed Markdown---is primarily a
language-side problem. Freezing the encoder also prevents drift in the
perception representations while the model adapts to the harder
serialization objective.

At convergence, Stage~2 produces fluent Markdown that is locally correct
on the majority of inputs. Sequence-level failures---unclosed tags,
inconsistent table widths, occasional heading-level skips---persist
because the cross-entropy objective cannot directly penalize them. These
are the failure modes Stage~3 is designed to address.

\subsection{Stage 3: Multi-Reward Refinement with GDPO}
\label{sec:stage3}

\paragraph{From SFT to multi-reward RL.} SFT minimizes a token-level
likelihood and cannot directly express sequence-level constraints such as
closed tags, consistent table shape, or valid heading hierarchy. We make
these constraints explicit through four rule-based rewards and optimize
them with GDPO \citep{liu2026gdpo}, which preserves per-dimension signal by
normalizing each reward independently within a rollout group; in contrast,
plain GRPO \citep{shao2024deepseekmath} normalizes only the summed reward
and collapses advantages across rollouts that differ along
\emph{different} reward dimensions.

\subsubsection{Reward Functions}
\label{sec:rewards}

All four rewards are defined over a rollout $o$ with text output $\hat{y}$
and ground truth $y^{\star}$. Each is normalized to $[0, 1]$ and computed
by a deterministic Python pipeline; we do not train an auxiliary reward
model.

\paragraph{(1) Text accuracy.} We strip Markdown and HTML markup from both
prediction and target, collapse whitespace, and compute one minus the
normalized Levenshtein distance \citep{levenshtein1966binary}:
\begin{equation}
\Rtext(\hat{y}, y^{\star}) \;=\; 1 - \frac{\Lev\!\left(\Pi(\hat{y}),\, \Pi(y^{\star})\right)}
{\max\!\left(|\Pi(\hat{y})|,\, |\Pi(y^{\star})|\right)},
\label{eq:r-text}
\end{equation}
where $\Pi(\cdot)$ is the strip-markup projection.

\paragraph{(2) Formula syntax.} For each predicted formula $\hat{f}_k$, we
verify that it compiles under KaTeX and evaluate its visual equivalence to
the matched target via Character Detection Matching
\citep{ouyang2412omnidocbench}:
\begin{equation}
\Rformula(\hat{y}, y^{\star}) \;=\; \frac{1}{K} \sum_{k=1}^{K} \Big[
  \alpha\, \mathbb{1}\!\left[\texttt{compile}(\hat{f}_k)\right]
  + (1 - \alpha)\, \mathrm{CDM}(\hat{f}_k, f^{\star}_k) \Big],
\label{eq:r-formula}
\end{equation}
with $\alpha = 0.3$. The asymmetric weighting reflects that successful
compilation is a necessary but weak property, whereas visual equivalence
more directly captures human-perceived correctness. When neither $\hat{y}$
nor $y^{\star}$ contains any formula, we set $\Rformula = 1$ by convention.

\paragraph{(3) Table integrity.} Because tables are HTML throughout
training, $\Rtable$ is defined directly against the HTML grammar:
\begin{equation}
\Rtable(\hat{y}, y^{\star}) \;=\; \beta\, S_{\text{shape}}^{\text{HTML}}(\hat{y}, y^{\star})
  + (1 - \beta)\, \mathrm{TEDS}(\hat{y}, y^{\star}),
\label{eq:r-table}
\end{equation}
where $\mathrm{TEDS}$ is the Tree-Edit-Distance Similarity
\citep{zhong2020image} computed on the parsed table tree, and the
shape-consistency term is the product of three checks:
\begin{equation}
S_{\text{shape}}^{\text{HTML}}(\hat{y}, y^{\star}) \;=\;
\underbrace{\mathbb{1}\!\left[\text{well-formed}(\hat{y})\right]}_{\text{tags close and nest}}
\cdot
\underbrace{\mathbb{1}\!\left[\text{cells-consistent}(\hat{y})\right]}_{\text{effective row widths agree}}
\cdot
\underbrace{\exp\!\left(-\gamma\, |N_{\text{row}}(\hat{y}) - N_{\text{row}}(y^{\star})|\right)}_{\text{row-count match}}.
\label{eq:r-table-shape}
\end{equation}
``Well-formed'' is decided by parsing $\hat{y}$ with \texttt{lxml.html} in
strict mode; failure scores zero. ``Cells-consistent'' computes the
effective row width
$W(r) = \sum_{c \in \text{cells}(r)} \texttt{colspan}(c)$, after adjusting
for active \texttt{rowspan}s, and requires $W(r) = W(r')$ for all row
pairs $r, r'$. This criterion is more permissive than direct column
counting in that it admits merged cells, yet stricter than mere agreement
on the number of rows in that it forbids implicitly truncated rows.
Defaults: $\beta = 0.4$, $\gamma = 0.1$. As boundary cases, if $\hat{y}$
contains no \texttt{<table>} while $y^{\star}$ does, $\Rtable = 0$; if
neither contains a table, $\Rtable = 1$.

\paragraph{(4) Structural closure.} Let $\mathcal{T}$ be the union of
Markdown pairs and HTML table tags:
\(
\mathcal{T} = \{\texttt{**}, \texttt{\_\_}, \texttt{\$\$}, \texttt{`}\}
\cup \{\texttt{<table>}, \texttt{<thead>}, \texttt{<tbody>}, \texttt{<tr>}, \texttt{<td>}, \texttt{<th>}\}.
\)
Then
\begin{equation}
\Rstruct(\hat{y}) \;=\; \left[ 1 - \frac{1}{|\mathcal{T}|}
\sum_{\tau \in \mathcal{T}} \frac{|N_{\text{open}}(\tau; \hat{y}) - N_{\text{close}}(\tau; \hat{y})|}
{N_{\text{open}}(\tau; \hat{y}) + N_{\text{close}}(\tau; \hat{y}) + \epsilon} \right]
\cdot \mathbb{1}\!\left[\text{heading-hierarchy-valid}(\hat{y})\right],
\label{eq:r-struct}
\end{equation}
where the multiplicative gate fires when heading depth jumps illegally
(\eg{} \verb|#| followed directly by \verb|###|) or list indentation is
malformed. $\Rstruct$ and $\Rtable$ overlap intentionally: $\Rstruct$ is
inexpensive and coarse-grained, providing useful gradient early in RL
training, when $\Rtable$ remains near zero on most rollouts and offers
little signal.

\paragraph{(5) Conditioned rewards.} The four rewards differ in their
susceptibility to gaming: an empty table is trivially well-formed, and
an output with no formulas trivially compiles. Following
\citet{liu2026gdpo}, we gate $\Rstruct, \Rformula, \Rtable$ on $\Rtext$:
\begin{equation}
\tilde{R}_{\bullet} \;=\; R_{\bullet}\, \mathbb{1}\!\left[\Rtext \geq \tau_{\text{text}}\right],
\qquad \tau_{\text{text}} = 0.7.
\label{eq:cond-reward}
\end{equation}

\subsubsection{Policy Update with GDPO}
\label{sec:gdpo}

For each prompt $I^{(i)}$ we sample $G$ rollouts
$\{o^{(i,j)}\}_{j=1}^{G}$ from $\pi_{\theta_{\text{old}}}$ and compute the
four (possibly conditioned) rewards $r_k^{(i,j)}$,
$k \in \{\text{text, formula, table, struct}\}$. The defining feature of
GDPO is to standardize \emph{per reward dimension} within the group, then
aggregate across dimensions and rescale across the batch $\mathcal{B}$:
\begin{equation}
A_k^{(i,j)} = \frac{r_k^{(i,j)} - \mu_k^{(i)}}{\sigma_k^{(i)} + \epsilon},
\qquad
A_{\text{sum}}^{(i,j)} = \sum_k w_k\, A_k^{(i,j)},
\qquad
\hat{A}^{(i,j)} = \frac{A_{\text{sum}}^{(i,j)} - \mu_{\mathcal{B}}}{\sigma_{\mathcal{B}} + \epsilon},
\label{eq:gdpo-adv}
\end{equation}
where $\mu_k^{(i)}, \sigma_k^{(i)}$ denote the within-group mean and
standard deviation of reward $k$. The per-reward step preserves the
gradient signal of each reward dimension that would otherwise be lost
when rewards are first summed and then normalized; the batch-level
rescaling keeps the effective learning rate stable as the number of
reward dimensions varies. We set the weights to
$w_{\text{text}} : w_{\text{formula}} : w_{\text{table}} : w_{\text{struct}}
= 1.0 : 0.8 : 0.8 : 0.5$, prioritizing text accuracy over structural
closure---consistent with the conditioning gate in
Eq.~\eqref{eq:cond-reward}.

The policy is then updated by maximizing the standard PPO clipped surrogate
\citep{schulman2017proximal} with $\hat{A}^{(i,j)}$ in place of the usual
advantage, regularized by a KL term
$\beta_{\KL}\, \KL(\pi_\theta \,\|\, \pi_{\text{ref}})$ that anchors
$\pi_\theta$ to the frozen Stage~2 checkpoint $\pi_{\text{ref}}$.

\subsubsection{Anti-Reward-Hacking in a Single-Pass Pipeline}
\label{sec:antihack}

We train Stages~2 and~3 in a single linear pass: GDPO takes over once
Stage~2 SFT converges, and remains the sole objective for the remainder of
training. An alternative design---alternating short rounds of SFT and RL
with hard-case mining in between, as in FireRed-OCR
\citep{wu2026firered}---is known to mitigate reward hacking but at the
cost of a more elaborate pipeline. We instead rely on three mutually
reinforcing mechanisms:

\begin{description}[leftmargin=1.6em, itemsep=0.25em, topsep=0.3em]
  \item[(i) Conditioned rewards.] Equation~\eqref{eq:cond-reward} forces text
    fidelity above $\tau_{\text{text}}$ before any structural reward fires,
    so degenerate solutions---empty tables, missing formulas---cannot
    accumulate reward.
  \item[(ii) KL anchor to the SFT checkpoint.] The KL term
    $\beta_{\KL}\, \KL(\pi_\theta \,\|\, \pi_{\text{ref}})$ introduced in
    \Cref{sec:gdpo} prevents the policy from drifting away from the
    Stage~2 distribution, preserving recognition capabilities that the RL
    objective alone does not explicitly enforce \citep{liu2025dler}.
  \item[(iii) Weight ordering.] With $w_{\text{text}}$ the largest
    aggregation weight, the policy gradient is biased toward text accuracy
    even after standardization.
\end{description}

\paragraph{Visual encoder freezing.} The visual encoder remains frozen
throughout Stage~3, continuing the setting introduced in Stage~2; only the
language model and the cross-modal projector are updated. Backpropagating
RL gradients through the visual encoder is particularly unstable in
practice, and freezing it further reduces per-rollout memory usage, which
enables a larger rollout group $G$ within a fixed memory budget.

==> method_v2.tex <==
% This file is intended to be included from `paper.tex` via \input.

\providecommand{\etal}{et al.}
\providecommand{\argmax}{\operatornamewithlimits{arg\,max}}
\providecommand{\Lev}{\operatorname{Lev}}
\providecommand{\KL}{\operatorname{KL}}
\providecommand{\Rtext}{R_{\text{text}}}
\providecommand{\Rformula}{R_{\text{formula}}}
\providecommand{\Rtable}{R_{\text{table}}}
\providecommand{\Rstruct}{R_{\text{struct}}}

\section{Methodology}
\label{sec:method}

We formulate document parsing as an end-to-end image-to-Markdown generation problem. Given a page image $I \in \mathbb{R}^{H \times W \times 3}$, the model $\pi_\theta$ autoregressively predicts a token sequence $y = (y_1, \dots, y_T)$ over a restricted Markdown vocabulary. The vocabulary covers plain text, hierarchical headings, lists, tables in HTML, display and inline \LaTeX{} formulas, and an implicit reading order among these elements.

Training proceeds in three stages with a shared objective. Let $\mathcal{D}$ denote the training distribution and $y^{\star}$ the ground-truth Markdown for image $I$. We optimize:

\begin{equation}
  \pi^{\star}
  = \arg\max_{\theta}\;
  \mathbb{E}_{(I,\, y^{\star}) \sim \mathcal{D}}
    \bigl[\log \pi_{\theta}(y^{\star} \mid I)\bigr]
  + \lambda\,
  \mathbb{E}_{I \sim \mathcal{D}}
    \bigl[\mathcal{R}\bigl(\pi_{\theta}(I)\bigr)\bigr].
  \label{eq:overall}
\end{equation}

where $\mathcal{R}(\cdot)$ is the rule-based reward defined in \Cref{sec:stage3}. In Stages1--2 we set $\lambda = 0$ and maximize only the supervised likelihood; in Stage3 we set $\lambda > 0$ and add reward optimization with GDPO. All stages use the same backbone, initialized from Qwen3-VL-2B-Instruct \citep{qwen3vl2025}.

\subsection{Training Pipeline}
\label{sec:overview}

A straightforward baseline is to fine-tune a strong vision--language model (VLM) on \textit{(page image, full Markdown)} pairs in a single step. In preliminary experiments, this recipe consistently underperforms for two reasons.

\textbf{Structural hallucination.}
The model often produces tables with inconsistent row widths, unmatched \texttt{\$\$} delimiters, and HTML tags that are opened but not closed.
Token-level cross-entropy does not directly penalize such errors, the loss can be small even when the decoded Markdown is structurally ill-formed.

\textbf{Gradient interference.}
Learning to locate glyphs, recognize their content, and serialize the page in Markdown imposes competing gradient signals.
As a result, accuracy on long-tail content such as rare formulas and complex table layouts degrades markedly.

These findings align with previous observations on document OCR systems \citep{fireredocr2025} and motivate decoupling perception, composition, and refinement before end-to-end integration.
Consequently, training follows the three-stage pipeline illustrated in \Cref{fig:three_stage_pipeline}.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/method.jpg}
    \caption{Overview of the proposed three-stage training pipeline for document-to-Markdown parsing. Stage~1 performs multi-task pre-alignment on text spotting, formula recognition, table recognition, and layout analysis to build fine-grained visual and structural perception. Stage~2 specializes the model with end-to-end supervised fine-tuning on normalized page-to-Markdown pairs. Stage~3 further refines the policy with GDPO using rule-based rewards for text fidelity, formula correctness, table integrity, and structural closure.}
    \label{fig:three_stage_pipeline}
\end{figure}

\subsection{Stage 1: Multi-task Pre-alignment}
\label{sec:stage1}

General-purpose VLMs typically encode only a coarse document prior: web-scale pretraining does not emphasize the fine-grained pixel-to-character alignment required for OCR.
We jointly optimizes four complementary objectives through a shared network.
Tasks are distinguished by different prompts, without task-specific heads \citep{bai2023qwen, chen2024internvl}.The four tasks are defined below:

\paragraph{Text spotting}
Given a text image and the prompt token \texttt{<spot>}, the model decodes sequences of the form
\[
  \texttt{<|box\_start|>(x1,y1),(x2,y2)<|box\_end|>text\_content},
\]
following the coordinate-token convention of Qwen-VL \citep{bai2023qwen}.
Spotting is the most demanding subtask for visual perception: the model must localize text regions, transcribe their content, and emit pixel-accurate boxes within a single autoregressive stream.
It provides the foundation for subsequent layout-aware supervision.

\paragraph{Formula recognition}
The input is either a cropped formula patch or a full page with a region-of-interest prompt; the target is a normalized \LaTeX{} string covering inline, display, and multi-line expressions.

\paragraph{Table recognition}
Given an image of a cropped table, the target is a normalized HTML table, because \texttt{rowspan} and \texttt{colspan} are native to HTML and a single markup grammar simplifies the structural reward in Stage~3 (\Cref{sec:stage3}).
\[
    \verb|<table><tr><td>...</td></tr></table>|.
\]

\paragraph{Layout analysis}
Given a full page and the prompt token \texttt{<layout>}, the model outputs a reading-order sequence of region boxes, each paired with a category from
\{\textit{title, text, table, figure, formula, footer, $\dots$}\}:
\[
  \texttt{<|box\_start|>(x1,y1),(x2,y2)<|box\_end|><type>title</type>}.
\]

\medskip
The four tasks form two complementary groups.
Spotting and layout provide global spatial supervision over the full page; formula and table recognition provide local structural supervision within their content domains.
Together, these signals encourage the shared visual encoder to capture both page-level geometry and region-level structure. 
The train dataset in Stage~1 is
$\mathcal{D}_{\text{S1}} = \mathcal{D}_{\text{spot}} \cup \mathcal{D}_{\text{formula}} \cup \mathcal{D}_{\text{table}} \cup \mathcal{D}_{\text{layout}}$.
We minimize the standard auto-regressive cross-entropy.
\begin{equation}
  \mathcal{L}_{\text{S1}}(\theta)
  = -\mathbb{E}_{(I, c, y) \sim \mathcal{D}_{\text{S1}}}
    \left[
      \sum_{t=1}^{|y|} \log \pi_{\theta}(y_t \mid y_{<t}, I, c)
    \right],
  \label{eq:l-stage1}
\end{equation}
where $c \in \{\texttt{<spot>}, \texttt{<formula>}, \texttt{<table>}, \texttt{<layout>}\}$ denotes the task-routing prompt.

After Stage~1, the visual encoder encodes glyph-level text, layout, and formula/table structure, so Stage~2 can focus on page-level Markdown serialization rather than reacquiring low-level perception.

\subsection{Stage 2: End-to-End Document Parsing}
\label{sec:stage2}

In this stage, optimization focuses on end-to-end composition: a single conditional mapping from a page image to a Markdown transcript that preserves all page content.
The dominant difficulty at this stage is structural well-formedness---closed tags, consistent heading depth, and properly delimited mathematics.

Let $\mathcal{D}_{\text{S2}} = \{(I^{\text{page}}_i, M^{\star}_i)\}_{i=1}^{N_2}$.
Ground-truth Markdown $M^{\star}$ is obtained through a strict normalization pipeline with the following invariants:
\begin{itemize}[leftmargin=1.4em, itemsep=0.15em, topsep=0.3em]
  \item Display mathematics uses \verb|$$ ... $$|; inline mathematics uses \verb|$ ... $|.
  \item All tables are represented in HTML, including those with merged cells, so that table rewards can be applied to a single markup grammar in Stage~3.
  \item Reading order follows visual layout: on multi-column pages, columns are emitted left to right, with each column completed before advancing.
  \item Heading depth is encoded by \verb|#|, \verb|##|, and \verb|###| without skipped levels (e.g., no transition from \verb|#| directly to \verb|###|).
\end{itemize}

The training objective is
\begin{equation}
  \mathcal{L}_{\text{S2}}(\theta)
  = -\mathbb{E}_{(I^{\text{page}}, M^{\star}) \sim \mathcal{D}_{\text{S2}}}
    \left[
      \sum_{t=1}^{|M^{\star}|}
        \log \pi_{\theta}\!\left(
          M^{\star}_t \mid M^{\star}_{<t}, I^{\text{page}}
        \right)
    \right].
  \label{eq:l-stage2}
\end{equation}

Training initializes from the Stage~1 checkpoint.
The visual encoder is frozen for all subsequent stages, only the language model and the cross-modal projector are updated.
Freezing the encoder further limits representation drift during adaptation to the harder serialization objective.

At convergence, Stage~2 yields fluent and locally accurate Markdown on most inputs.
Due to cross-entropy does not directly penalize global validity, sequence-level errors nevertheless remain like unclosed tags, inconsistent table row widths, and occasional heading-level skips.

\subsection{Stage 3: Multi-Reward Refinement with GDPO}
\label{sec:stage3}

SFT minimizes token-level likelihood and cannot directly enforce sequence-level constraints such as closed tags, consistent table shape, or valid heading hierarchy.
These constraints are encoded as four rule-based rewards and optimized with GDPO \citep{liu2026gdpo}, which normalizes each reward dimension independently within a rollout group and thereby preserves per-dimension signal.
By contrast, standard GRPO \citep{shao2024deepseekmath} normalizes only the summed reward, which can collapse advantages across rollouts that differ along distinct reward dimensions.

\subsubsection{Reward Functions}
\label{sec:rewards}

All rewards are computed on a rollout $o$ with model output $\hat{y}$ and ground truth $y^{\star}$.
Each reward is mapped to $[0,1]$ by a deterministic Python evaluator and no auxiliary reward model is trained.

\paragraph{(1) Text accuracy}
Markdown and HTML markup are stripped from both prediction and target, whitespace is collapsed, and one minus the normalized Levenshtein distance \citep{levenshtein1966binary} is taken:
\begin{equation}
  \Rtext(\hat{y}, y^{\star})
  = 1 - \frac{
      \Lev\!\left(\Pi(\hat{y}),\, \Pi(y^{\star})\right)
    }{
      \max\!\left(|\Pi(\hat{y})|,\, |\Pi(y^{\star})|\right)
    },
  \label{eq:r-text}
\end{equation}
where $\Pi(\cdot)$ denotes the strip-markup projection.

\paragraph{(2) Formula syntax}
For each predicted formula $\hat{f}_k$, compilability under KaTeX is checked and visual equivalence to the matched reference is scored with Character Detection Matching (CDM) \citep{unimernet2024}:
\begin{equation}
  \Rformula(\hat{y}, y^{\star})
  = \frac{1}{K} \sum_{k=1}^{K}
    \Big[
      \alpha\, \mathbb{1}\!\left[\texttt{compile}(\hat{f}_k)\right]
      + (1 - \alpha)\, \mathrm{CDM}(\hat{f}_k, f^{\star}_k)
    \Big],
  \label{eq:r-formula}
\end{equation}
with $\alpha = 0.3$.
The weighting is asymmetric because successful compilation is necessary yet weakly indicative of correctness, whereas CDM more closely reflects human-perceived formula quality.
When neither $\hat{y}$ nor $y^{\star}$ contains a formula, $\Rformula = 1$ by convention.

\paragraph{(3) Table integrity}
Because tables are HTML throughout training, $\Rtable$ is defined directly on the HTML representation:
\begin{equation}
  \Rtable(\hat{y}, y^{\star})
  = \beta\, S_{\text{shape}}^{\text{HTML}}(\hat{y}, y^{\star})
    + (1 - \beta)\, \mathrm{TEDS}(\hat{y}, y^{\star}),
  \label{eq:r-table}
\end{equation}
where $\mathrm{TEDS}$ is Tree-Edit-Distance Similarity \citep{zhong2020image} on the parsed table trees.
The shape term factorizes into three checks:
\begin{equation}
  S_{\text{shape}}^{\text{HTML}}(\hat{y}, y^{\star})
  = \underbrace{\mathbb{1}\!\left[\text{well-formed}(\hat{y})\right]}_{\text{tags close and nest}}
    \cdot
    \underbrace{\mathbb{1}\!\left[\text{cells-consistent}(\hat{y})\right]}_{\text{uniform effective row widths}}
    \cdot
    \underbrace{\exp\!\left(-\gamma\, \left|N_{\text{row}}(\hat{y}) - N_{\text{row}}(y^{\star})\right|\right)}_{\text{row-count match}}.
  \label{eq:r-table-shape}
\end{equation}
Well-formedness is verified by parsing $\hat{y}$ with \texttt{lxml.html} in strict mode and parse failure yields zero contribution.
Cell consistency computes the effective row width
$W(r) = \sum_{c \in \text{cells}(r)} \texttt{colspan}(c)$ after accounting for active \texttt{rowspan} spans, and requires $W(r) = W(r')$ for all row pairs $(r,r')$.
The criterion is looser than naive column counting in the presence of merged cells, but tighter than row-count-only checks in that implicitly truncated rows are rejected.
We set $\beta = 0.4$ and $\gamma = 0.1$ throughout.
If $\hat{y}$ contains no \texttt{<table>} while $y^{\star}$ does, $\Rtable = 0$; if neither contains a table, $\Rtable = 1$.

\paragraph{(4) Structural closure}
Let $\mathcal{T}$ denote the set of paired Markdown delimiters and HTML table tags,
\(
\mathcal{T} = \{\texttt{**}, \texttt{\_\_}, \texttt{\$\$}, \texttt{`}\}
\cup \{\texttt{<table>}, \texttt{<thead>}, \texttt{<tbody>}, \texttt{<tr>}, \texttt{<td>}, \texttt{<th>}\}.
\)
Then
\begin{equation}
  \Rstruct(\hat{y})
  = \left[
      1 - \frac{1}{|\mathcal{T}|}
      \sum_{\tau \in \mathcal{T}}
        \frac{
          \left|N_{\text{open}}(\tau; \hat{y}) - N_{\text{close}}(\tau; \hat{y})\right|
        }{
          N_{\text{open}}(\tau; \hat{y}) + N_{\text{close}}(\tau; \hat{y}) + \epsilon
        }
    \right]
    \cdot \mathbb{1}\!\left[\text{heading-hierarchy-valid}(\hat{y})\right],
  \label{eq:r-struct}
\end{equation}
where the multiplicative gate enforces legal heading depth (e.g., no jump from \verb|#| to \verb|###|) and valid list indentation.
$\Rstruct$ and $\Rtable$ overlap by design: $\Rstruct$ is inexpensive and coarse, supplying early RL signal when $\Rtable$ remains near zero on most rollouts.

\paragraph{Reward conditioning}
The four rewards differ in susceptibility to gaming---empty tables are trivially well-formed, and formula-free outputs trivially compile.
Following \citet{liu2026gdpo}, $\Rstruct$, $\Rformula$, and $\Rtable$ are gated on text fidelity:
\begin{equation}
  \tilde{R}_{\bullet}
  = R_{\bullet}\, \mathbb{1}\!\left[\Rtext \geq \tau_{\text{text}}\right],
  \qquad \tau_{\text{text}} = 0.7.
  \label{eq:cond-reward}
\end{equation}

\subsubsection{Policy Update with GDPO}
\label{sec:gdpo}

For each prompt $I^{(i)}$, $G$ rollouts $\{o^{(i,j)}\}_{j=1}^{G}$ are sampled from $\pi_{\theta_{\text{old}}}$, and the four (possibly conditioned) rewards $r_k^{(i,j)}$ are evaluated for
$k \in \{\text{text, formula, table, struct}\}$.
GDPO standardizes each reward dimension within the group, aggregates across dimensions, and rescales over the minibatch $\mathcal{B}$:
\begin{equation}
  A_k^{(i,j)} = \frac{r_k^{(i,j)} - \mu_k^{(i)}}{\sigma_k^{(i)} + \epsilon},
  \qquad
  A_{\text{sum}}^{(i,j)} = \sum_k w_k\, A_k^{(i,j)},
  \qquad
  \hat{A}^{(i,j)} = \frac{A_{\text{sum}}^{(i,j)} - \mu_{\mathcal{B}}}{\sigma_{\mathcal{B}} + \epsilon},
  \label{eq:gdpo-adv}
\end{equation}
where $\mu_k^{(i)}$ and $\sigma_k^{(i)}$ are the within-group mean and standard deviation of reward $k$.
Per-reward normalization retains gradient signal that would be lost if rewards were summed before normalization; batch-level rescaling stabilizes the effective learning rate as the reward dimensionality changes.
Aggregation weights are set to
$w_{\text{text}} : w_{\text{formula}} : w_{\text{table}} : w_{\text{struct}} = 1.0 : 0.8 : 0.8 : 0.5$,
prioritizing text accuracy over structural closure and aligning with the conditioning gate in \eqref{eq:cond-reward}.

The policy is updated by maximizing the clipped PPO surrogate \citep{schulman2017proximal} with $\hat{A}^{(i,j)}$ substituted for the usual advantage, regularized by
$\beta_{\KL}\, \KL(\pi_{\theta} \,\|\, \pi_{\text{ref}})$,
which anchors $\pi_{\theta}$ to the frozen Stage~2 checkpoint $\pi_{\text{ref}}$.

